Finding Most Shattering Minimum Vertex Cuts of Polylogarithmic Size in Near-Linear Time

We show the first near-linear time randomized algorithms for listing all minimum vertex cuts of polylogarithmic size that separate the graph into at least three connected components (also known as shredders) and for finding the most shattering one, i.e., the one maximizing the number of connected components. Our algorithms break the quadratic time bound by Cheriyan and Thurimella (STOC'96) for both problems that has stood for more than two decades. Our work also removes a bottleneck to near-linear time algorithms for the vertex connectivity augmentation problem (Jordan '95). Note that it is necessary to list only minimum vertex cuts that separate the graph into at least three components because there can be an exponential number of minimum vertex cuts in general. To obtain near-linear time algorithms, we have extended techniques in local flow algorithms developed by Forster et al. (SODA'20) to list shredders on a local scale. We also exploit fast queries to a pairwise vertex connectivity oracle subject to vertex failures (Long and Saranurak FOCS'22, Kosinas ESA'23). This is the first application of connectivity oracles subject to vertex failures to speed up a static graph algorithm.

==> src/5-balanced.tex <==
\section{The General Strategy} \label{sec:general-strategy}
Recall that a $k$-shredder $S$ has partition $(C, \R)$ if $C$ is the largest component of $G \sm S$ by volume and $\R$ is the set of remaining components. In short, we introduce a notion of \textit{how} a $k$-shredder $S$ separates $G$ in terms of the ratio between the largest component of $G \sm S$ and the remaining components of $G \sm S$, namely the ratio between $\vol(C)$ and $\vol(\mc{R})$. Recall the following definition.

\defbalanced*

Our algorithm for listing $k$-shredders has two cases: one for the balanced ones and the unbalanced ones. Recall \Cref{def:balanced}.\thatchaphol{I feel we do not need this section.  We already give a high-level of Section 5.1 in Section 2.3 (we can add one more sentence like ``by sampling $O(k \log n)$ pairs of edges, we will hit $C$ and $\R$ as the smaller side has volume at least $m/k$.  The detailed calculation can be moved to \Cref{sec:all-k-shredders}.
We can also move some discussion in Section 5.2 to Section 2.5. I kind of want to get to the cool stuff (Sections 7 and 7 quickly).}


\subsection{Unbalanced \fmt{$k$}--Shredders}
We now turn our attention to unbalanced $k$-shredders. Fix an unbalanced $k$-shredder $S$ with partition $(C, \R)$. Unfortunately, the same probabilistic approach we used to prove \Cref{lem:balanced} does not work here. Specifically, if we sample two vertices, the probability that they are in different components of $G \sm S$ can be arbitrarily small. What this dilemma implies is that we must spend at least a linear amount of time just to collect samples. More critically, we must spend a sublinear amount of time processing an \textit{individual} sample to make any meaningful improvement. This time constraint rules out the possibility of calling $\SHR(\cdot, \cdot)$ per sample. Instead, we must develop a \textit{localized} version of $\SHR(\cdot, \cdot)$ that spends time relative to a parameter of our choice, instead of a global value such as $m$ or $n$.

In detail, consider an unbalanced $k$-shredder $S$ with partition $(C, \R)$. Observe that there must exist a power of two $2^i$ such that $2^{i-1} < \vol(\R) \leq 2^i$. If we sample $\tO(m/2^i)$ edges $(x, y)$, we will sample a vertex $x \in \R$ with high probability due to the classic hitting set lemmas. The goal is to spend only $\tO(\poly(k) \cdot 2^i)$ time processing each sample to list $S$. Suppose that such a local algorithm exists. Although we do not know the exact power of two $2^i$, we know that $\vol(\R) < \frac{m}{k}$. Hence, we can simply try all powers of two up to $\frac{m}{k}$. This gives us the near-linear runtime bound:
\begin{align*}
    \sum_{i=0}^{\lceil \log \frac{m}{k} \rceil} \tO\left(\frac{m}{2^i}\right) \cdot \tO(\poly(k) \cdot 2^i) & = \sum_{i=0}^{\lceil \log \frac{m}{k} \rceil} \tO(\poly(k) \cdot m) \\
    & = \tO(\poly(k) \cdot m).
\end{align*}
In the following sections, we show the localized framework.

